Template-based Gravitational-Wave Echoes Search Using Bayesian Model Selection

The ringdown of the gravitational-wave signal from a merger of two black holes has been suggested as a probe of the structure of the remnant compact object, which may be more exotic than a black hole. It has been pointed out that there will be a train of echoes in the late-time ringdown stage for different types of exotic compact objects. In this paper, we present a template-based search methodology using Bayesian statistics to search for echoes of gravitational waves. Evidence for the presence or absence of echoes in gravitational-wave events can be established by performing Bayesian model selection. The Occam factor in Bayesian model selection will automatically penalize the more complicated model that echoes are present in gravitational-wave strain data because of its higher degree of freedom to fit the data. We find that the search methodology was able to identify gravitational-wave echoes with Abedi et al.'s echoes waveform model about 82.3% of the time in simulated Gaussian noise in the Advanced LIGO and Virgo network and about 61.1% of the time in real noise in the first observing run of Advanced LIGO with $\geq 5\sigma$ significance. Analyses using this method are performed on the data of Advanced LIGO's first observing run, and we find no statistical significant evidence for the detection of gravitational-wave echoes. In particular, we find $<1\sigma$ combined evidence of the three events in Advanced LIGO's first observing run. The analysis technique developed in this paper is independent of the waveform model used, and can be used with different parametrized echoes waveform models to provide more realistic evidence of the existence of echoes from exotic compact objects.

==> echoes_acronyms.tex <==
\newacronym{GW}{GW}{gravitational-wave}
\newacronym{LIGO}{LIGO}{Laser Interferometer Gravitational-wave Observatory}
\newacronym{ECO}{ECO}{exotic compact object}
\newacronym{IMR}{IMR}{inspiral-merger-ringdown}
\newacronym{IMRE}{IMRE}{inspiral-merger-ringdown-echo}
\newacronym{MLE}{MLE}{maximum likelihood estimator}
\newacronym{MAP}{MAP}{maximum a posteriori estimator}
\newacronym{O1}{O1}{the first observing run}
\newacronym{ROC}{ROC}{receiver operating characteristic}

==> echoes_numbers.tex <==
\newcommand{\GaussianEfficiencyPercentage}{82.3}
\newcommand{\GaussianEfficiencyDecimal}{0.823}

% FIXME Not a particularly elegant way of writing O1, but it seems that LaTeX marco name only allows letters...
\newcommand{\OOneEfficiencyPercentage}{61.1}
\newcommand{\OOneEfficiencyDecimal}{0.611}

%\newcommand{\GaussianOneSigma}{-0.945}
%\newcommand{\GaussianTwoSigma}{-0.413}
%\newcommand{\GaussianThreeSigma}{1.093}
%\newcommand{\GaussianFourSigma}{1.531}
%\newcommand{\GaussianFiveSigma}{1.849}
\newcommand{\GaussianOneSigma}{-0.9}
\newcommand{\GaussianTwoSigma}{-0.4}
\newcommand{\GaussianThreeSigma}{1.1}
\newcommand{\GaussianFourSigma}{1.5}
\newcommand{\GaussianFiveSigma}{1.9}

%\newcommand{\OOneOneSigma}{0.075}
%\newcommand{\OOneTwoSigma}{1.509}
%\newcommand{\OOneThreeSigma}{3.955}
%\newcommand{\OOneFourSigma}{5.355}
%\newcommand{\OOneFiveSigma}{5.689}
\newcommand{\OOneOneSigma}{0.1}
\newcommand{\OOneTwoSigma}{1.5}
\newcommand{\OOneThreeSigma}{4.0}
\newcommand{\OOneFourSigma}{5.4}
\newcommand{\OOneFiveSigma}{5.7}

\newcommand{\GaussianThreshold}{\GaussianFiveSigma}
\newcommand{\OOneThreshold}{\OOneFiveSigma}
